F-IDEs with Features and VCs Designed to Assist Human Reasoning When Verification Fails

This paper summarizes our efforts to aid human reasoning when verification fails through the use of two distinct Formalization Integrated Development Environments (F-IDEs) that we have developed. Both environments are modular and facilitate reasoning about the full behavior of object-based code. The first environment, referred to as the web-IDE, has been used for several years to teach aspects of formal specification and verification, including why and where verification conditions (VCs) arise and how to use them when verification fails. The second F-IDE, RESOLVE Studio, remains experimental, but is a more fully-fledged environment backed by a sequent-based VC generator that produces VCs with fewer extraneous givens. While the environments and VC generation techniques are necessarily language specific, the principles of alternative VC generation methods, F-IDE features, and observations about their impact on novices and experienced users are more generally applicable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{51}
\providecommand{\publicationstatus}{M. Gleirscher, J.v.d. Pol, J. Woodcock (Eds.):\\First Workshop on Applicable Formal Methods (AppFM 2021).\\
EPTCS 349, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.349.4}{10.4204/EPTCS.349.4}}
\pdfoutput=1

